Measurement of the average transverse momentum of forward prompt charged particles in $pp$ and $p\mathrm{Pb}$ collisions at $\sqrt{s_{NN}} = 5.02\; \mathrm{TeV}$

This letter presents the first measurements of the average transverse momentum of prompt charged particles in $pp$ and $p\mathrm{Pb}$ collisions as a function of collision multiplicity and pseudorapidity. The data were recorded at nucleon-nucleon centre-of-mass energy $\sqrt{s_{NN}} = 5.02\; \mathrm{TeV}$ with the LHCb experiment. The pseudorapidity dependence of the multiplicity distribution is also measured. The average transverse momentum results show a decreasing trend with pseudorapidity, more pronounced in high-multiplicity events, consistent with the collective behaviour of the produced matter. The measurements are reproduced by state-of-the-art (3+1D) hydrodynamic calculations, while saturation models are not compatible with the data.

==> LHCb/local-symbols-def.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Physics symbols
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Packages we need
\RequirePackage{xspace}

% More semantic name than texttt
\newcommand{\functor}[1]{\texttt{#1}\xspace}

% local
\def\avpt {\ensuremath{\langle p_T\rangle} \xspace}

% Yields 
\def\N{\ensuremath{N_{\mathrm{tracks}}}} % Used to indicate the number of prompt charged particles inside the acceptance

% Heavy ion
\def\pA   {\ensuremath{p\mathrm{Pb}}\xspace}
\def\Ap   {\ensuremath{\mathrm{Pb}p}\xspace}
\def\pp   {\ensuremath{pp}\xspace}
\def\Rppb {\ensuremath{\mathrm{R}_{p\mathrm{Pb}}}\xspace}
\def\Rpbp {\ensuremath{\mathrm{R}_{\mathrm{Pb}p}}\xspace}
\def\RFB {\ensuremath{\mathrm{R}_{\mathrm{FB}}}\xspace}
\def\RBF {\ensuremath{\mathrm{R}_{\mathrm{BF}}}\xspace}
\def\Rppbch {\ensuremath{\mathrm{R}_{p\mathrm{Pb}}^{ch}}\xspace}
\def\Rpbpch {\ensuremath{\mathrm{R}_{\mathrm{Pb}p}^{ch}}\xspace}
\def\YFBch {\ensuremath{Y^{ch}_{\mathrm{FB}}}\xspace}
\def\ghP {\ensuremath{\mathtt{GhostP}}\xspace} 
\def\clone {\ensuremath{\mathtt{IsClone}}\xspace}
\def\psIP {\ensuremath{\mathtt{pseudoIP}}\xspace}
\def\IP {\ensuremath{\mathtt{IP}}\xspace}
\def\sNN {\ensuremath{\sqrt{s_{\mathrm{NN}}}}\xspace}
\def\meanpt{\ensuremath{\langle p_\mathrm{T} \rangle}\xspace}
\def\meanptNch{\ensuremath{\langle p_\mathrm{T} \rangle (N_\mathrm{ch})}\xspace}
\def\meanptNcheta{\ensuremath{\langle p_\mathrm{T} \rangle (N_\mathrm{ch}^{\mathrm{acc}}, \eta)}\xspace}
\def\meanptNcorr{\ensuremath{\langle p_\mathrm{T} \rangle (N_\mathrm{corr})}\xspace}
\def\pt{\ensuremath{p_{\mathrm{T}}}\xspace}

% simulations
\def\epos     {\mbox{\textsc{Epos-lhc}}\xspace}
\def\hijing     {\mbox{\textsc{Hijing}}\xspace}

\def\ovtype {\ensuremath{\mathtt{OV\_type}}\xspace}

% occupancies
%% \def\velotr {\ensuremath{\mathtt{nVeloTracks}}\xspace}
\def\velotr {\ensuremath{N^\text{VELO}_\text{tracks}}\xspace}


\def\cems {\ensuremath{\mathrm{cms}}\xspace}
\def\Nvelo {\ensuremath{N_{\mathrm{VELO}}^{\mathrm{clusters}}}\xspace}
\def\Nspd {\ensuremath{N_{\mathrm{SPD}}^{\mathrm{Hits}}}\xspace}
\def\Nclus {\ensuremath{N_{\mathrm{VELO}}^{\mathrm{clusters}}}\xspace}

\def\etacms {\ensuremath{\eta_{\mathrm{cms}}}\xspace}

% Yields 
\def\Ntrack{\ensuremath{N_{\mathrm{track}}}\xspace} % Used to indicate the number of prompt charged particles inside the acceptance

% Multiplicity related quantities
\def\Ncand {\ensuremath{N_{\mathrm{cand}}^{\mathrm{acc}}}\xspace}
\def\Nch {\ensuremath{N_{\mathrm{ch}}^{\mathrm{acc}}}\xspace}
\def\Ncorr {\ensuremath{N_{\mathrm{corr}}}\xspace}
\def\Ngen {\ensuremath{N_{\mathrm{gen}}}\xspace}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Special text
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% Commenting for early drafts.
%\newcommand{\comment}[1]{
%\ifreview
	%\textit{\color{red}#1}
%\else
%\fi
%}


%% References
\newcommand{\Tabref}[1]{Tab.~\protect\ref{#1}}
\newcommand{\Tabrefs}[2]{Tabs.~\protect\ref{#1} and~\protect\ref{#2}}
\newcommand{\Figref}[1]{Fig.~\protect\ref{#1}}
\newcommand{\Figrefs}[2]{Figs.~\protect\ref{#1} and~\protect\ref{#2}}
\newcommand{\Figrange}[2]{Figs.~\protect\ref{#1} $-$~\protect\ref{#2}}
\newcommand{\Figrefsthree}[3]{Figs.~\protect\ref{#1},~\protect\ref{#2} and~\protect\ref{#3}}
\newcommand{\Secref}[1]{Sec.~\protect\ref{#1}}
\newcommand{\Secrefs}[2]{Secs.~\protect\ref{#1} and~\protect\ref{#2}}
\newcommand{\Secrefsthree}[3]{Secs.~\protect\ref{#1},~\protect\ref{#2} and~\protect\ref{#3}}
\newcommand{\Appref}[1]{App.~\protect\ref{#1}}
\newcommand{\Apprefs}[2]{Apps.~\protect\ref{#1} and~\protect\ref{#2}}
\newcommand{\Eqref}[1]{Eq.~\protect\ref{#1}}
\newcommand{\Eqrefs}[2]{Eqs.~\protect\ref{#1} and~\protect\ref{#2}}
\newcommand{\Eqrefsthree}[3]{Eqs.~\protect\ref{#1},~\protect\ref{#2} and~\protect\ref{#3}}
%% Luminosity macros
\newcommand{\lumisummary}{\ensuremath{\textit{1024}\invpb}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%
% Software
%%%%%%%%%%%%%%%%%%%%%%%%
\def\tesla   {\textsc{Tesla}\xspace}
\def\loki    {\textsc{LoKi}\xspace}
\def\pidcalib {\textsc{PIDCalib}\xspace}
\def\pythiaeight    {\textsc{Pythia8}\xspace}
\def\geantfour {\textsc{Geant4}\xspace}

% Track quality
\def\IP          {IP\xspace}
\def\ipchisqndof {\ensuremath{\mathrm{IP}\chisq/\mathrm{ndof}}\xspace}
\def\lnchisq     {\ensuremath{\log{\chisq}}\xspace}
\def\ipchisq     {\ensuremath{\chi^2_{\rm IP}}\xspace}
\def\lnipchisq   {\ensuremath{\ln{\chi^2_{\rm IP}}}\xspace}

% PID
\def\probnnk {\mathrm{ProbNN\ensuremath{k}}\xspace}

% LHCb trigger jargon
\def\tis    {TIS\xspace}
\def\tos    {TOS\xspace}
\def\tistos {\tis{}\tos{}\xspace}

\def\invmub{\ensuremath{\,\upmu\nospaceunit{b}^{-1}}\xspace}

